POINTREC: A Test Collection for Narrative-driven Point of Interest Recommendation

This paper presents a test collection for contextual point of interest (POI) recommendation in a narrative-driven scenario. There, user history is not available, instead, user requests are described in natural language. The requests in our collection are manually collected from social sharing websites, and are annotated with various types of metadata, including location, categories, constraints, and example POIs. These requests are to be resolved from a dataset of POIs, which are collected from a popular online directory, and are further linked to a geographical knowledge base and enriched with relevant web snippets. Graded relevance assessments are collected using crowdsourcing, by pooling both manual and automatic recommendations, where the latter serve as baselines for future performance comparison. This resource supports the development of novel approaches for end-to-end POI recommendation as well as for specific semantic annotation tasks on natural language requests.

==> sigir2021-poi-a1.tex <==
\section{Appendix}

\subsection{Sources of Information Needs}
\label{sec:app:infoneeds}

Table~\ref{tab:subreddits} presents the list of subreddits that were used for extracting information needs.

\begin{table}[h]
\caption{List of subreddits (suffixes following \texttt{http://reddit.com/r/}) and the corresponding number of information needs extracted.}
\vspace*{-\baselineskip}
\label{tab:subreddits}
\begin{tabular}{lr}
	\toprule	
	\textbf{Subreddit} & \textbf{\#InfoNeeds} \\
	\midrule
Amsterdam       &  6 \\
askTO           &  1 \\
Austin          &  1 \\
Austria         &  1 \\
berlin          &  3 \\
bologna         &  1 \\
britishcolumbia &  1 \\
Caen            &  1 \\
chicago         &  1 \\
Delaware        &  3 \\
Detroit         &  3 \\
geneva          &  1 \\
glendale        &  1 \\
Hamilton        &  1 \\
helsinki        &  3 \\
hiking          &  1 \\
JapanTravel     &  4 \\
Knoxville       &  1 \\
london          &  1 \\
madisonwi       &  1 \\
Madrid          &  1 \\
melbourne       &  1 \\
milwaukee       &  1 \\
mountainview    &  1 \\
nyc             &  1 \\
oslo            &  4 \\
paris           &  5 \\
Prague          &  1 \\
quebeccity      &  1 \\
raleigh         &  2 \\
rome            &  2 \\
Rotterdam       &  1 \\
rva             &  1 \\
SaltLakeCity    &  1 \\
SkyDiving       &  2 \\
solotravel      &  8 \\
Stavanger       &  2 \\
Switzerland     &  1 \\
Temecula        &  1 \\
Tennessee       &  1 \\
texas           &  1 \\
Tokyo           &  2 \\
Utah            &  1 \\
VictoriaBC      &  1 \\
wallawalla      &  1 \\
Washington      &  1 \\
Westchester     &  1 \\
wien            &  4 \\
zurich          &  2 \\
	\bottomrule
\end{tabular}
\vspace*{-\baselineskip}
\end{table}

\subsection{POI Collection}
\label{sec:app:poi}

A complete breakdown of the POI collection per country and per main category is shown in Tables~\ref{tab:poi:Country_Stats_data} and \ref{tab:poi:Category_Stats_data}, respectively.

\begin{table}[h]
 \caption{Breakdown of the POI collection per country.} 
 \begin{tabular}{l r r r}
 \toprule
 \textbf{Country} & \textbf{\#cities} & \textbf{\#POIs} & \textbf{Avg \#POI/city}\\
 \midrule
US & 404 & 315238 & 780.3 \\ 
DE & 397 & 187024 & 471.1 \\ 
CA & 123 & 34804 & 283.0 \\ 
JP & 205 & 30843 & 150.5 \\ 
ES & 117 & 23628 & 201.9 \\ 
FR & 54 & 22642 & 419.3 \\ 
GB & 35 & 18916 & 540.5 \\ 
AU & 15 & 8944 & 596.3 \\ 
AT & 250 & 8673 & 34.7 \\ 
NL & 112 & 8143 & 72.7 \\ 
IT & 17 & 7322 & 430.7 \\ 
CZ & 37 & 6432 & 173.8 \\ 
CH & 270 & 6080 & 22.5 \\ 
PT & 112 & 5959 & 53.2 \\ 
MX & 39 & 3617 & 92.7 \\ 
NO & 14 & 3183 & 227.4 \\ 
FI & 6 & 3134 & 522.3 \\ 
PL & 20 & 219 & 11.0 \\ 
BE & 10 & 132 & 13.2 \\ 
DK & 8 & 95 & 11.9 \\ 
AR & 1 & 4 & 4.0 \\ 
MY & 1 & 2 & 2.0 \\ 
TR & 1 & 1 & 1.0 \\ 
\bottomrule
\end{tabular}
\label{tab:poi:Country_Stats_data} 
\end{table}


 \begin{table}[h]
 \caption{Breakdown of the POI collection per main category.} 
 \begin{tabular}{l r}
 \toprule
 \textbf{Main Category} & \textbf{\#POIs} \\ 
 \midrule
	Restaurants and Food & 496403\\ 
	Active Life&89113\\ 
	Arts \& Entertainment&55122\\ 
	Nightlife&43175\\ 
	Event Planning \& Services & 3643\\ 
	Shopping & 2462 \\ 
	Public Services \& Government & 1686\\ 
	Hotels \& Travel& 1022\\ 
	Local Flavor & 648 \\ 
	Education & 368  \\
	Health \& Medical & 309 \\ 
	Beauty \& Spas & 202\\ 
	Local Services & 195\\ 
	Home Services & 169\\ 
	Religious Organizations & 147\\ 
	Professional Services & 122\\ 
	Automotive & 87\\ 
	Pets & 86\\  
	Financial Services & 57\\ 
	Mass Media & 19\\ 
\bottomrule
\end{tabular}
\label{tab:poi:Category_Stats_data}
\end{table}

\begin{figure}[b]
\scriptsize
\begin{verbatim}
{
    "query": {
      "bool": {
        "should": [
          {
            "multi_match": {
              "query": "Berlin",
              "fields": [
                "city",
                "city_from_postal"
              ]
            }
          },
          {
            "match": {
              "sub_categories": "Museums Art Galleries Castles"
            }
          },
          {
            "match": {
              "snippets": "monuments, museums, castles, art galleries"
            }
          },
          {
            "match": {
              "snippets": "Recommendations for attractions"
            }
          }
        ],
        "filter": {
          "match": {
            "country_code": "DE"
          }
        },
        "must": [
          {
            "match": {
              "main_category": "Arts & Entertainment"
            }
          }
        ]
      }
    }
  }
\end{verbatim}	
\caption{Example Elasticsearch query for Baseline 3.}
\label{fig:query}
\end{figure}

